Confident yet Concerned: Inconsistencies in Computing Students' Attitudes on Cybersecurity

Today's young adults are most immersed in technology, leading in feelings of powerlessness in managing online privacy across many platforms, and particularly susceptible to phishing attacks. This raises questions about their general, wide-ranging attitudes towards and management of cybersecurity. How do young, tech-savvy adults approach cybersecurity? We seek a better understanding of their cybersecurity knowledge, attitudes and experiences, in particular in addressing deceptive online communications. We surveyed a group of `lead users': computing university students (n = 236). By combining thematic analysis of open-ended responses with quantitative data, we provide insights into their experiences and perceptions. While students demonstrate reasonable cybersecurity awareness, their cybersecurity experiences vary, and inconsistencies exist around their practices, perceptions of responsibility, and support structures. Findings also reveal four key thematic tensions: 1) Computing students are knowledgeable yet have persistent incorrect beliefs, 2) They learn more about keeping safe from sources outside the classroom, 3) They have limited assistance and have fallen victim to cybercrime, and 4) Many are confident, yet others are concerned about their own safety and responsibility. Through cluster analysis of attitudes, we identify two groups, with one feeling less prepared, less confident, yet expressing a desire to learn more. Established measures of intentions and objective knowledge were correlated to preparedness. Self-efficacy correlated to confidence and predicted cluster membership.

==> Stats/cs.tex <==
CS: $\chi^2(1)=4.070$, $p=0.044$%


==> Stats/csexpl.tex <==
(CS: $N_{C1}=40, N_{C2}=44$; Non: $N_{C1}=39, N_{C2}=20$)%


==> Stats/gotvic.tex <==
WOM:: $\chi^2{1)=9.462$, $p=0.002$


==> Stats/spg.tex <==
SeBIS: $M_{C1}=54.0, M_{C2}=55.2$ $t(233.99) = -1.16$, $p = .123$, $d = -0.15$; Pew: $M_{C1}=5.3, M_{C2}=5.5$ $t(232.67) = -1.48$, $p = .071$, $d = -0.19$; GSE: $M_{C1}=39.4, M_{C2}=47.7$ $t(233.98) = -6.22$, $p < .001$, $d = -0.81$%

